Estimating Black Hole Masses in Active Galactic Nuclei Using the MgII 2800 Emission Line

We investigate the relationship between the linewidths of broad Mg II \lambda2800 and Hbeta in active galactic nuclei (AGNs) to refine them as tools to estimate black hole (BH) masses. We perform a detailed spectral analysis of a large sample of AGNs at intermediate redshifts selected from the Sloan Digital Sky Survey, along with a smaller sample of archival ultraviolet spectra for nearby sources monitored with reverberation mapping. Careful attention is devoted to accurate spectral decomposition, especially in the treatment of narrow-line blending and Fe II contamination. We show that, contrary to popular belief, the velocity width of Mg II tends to be smaller than that of Hbeta, suggesting that the two species are not cospatial in the broad-line region. Using these findings and recently updated BH mass measurements from reverberation mapping, we present a new calibration of the empirical prescriptions for estimating virial BH masses for AGNs using the broad Mg II and Hbeta lines. We show that the BH masses derived from our new formalisms show subtle but important differences compared to some of the mass estimators currently used in the literature.

==> full_table2.tex <==
\begin{deluxetable}{lccccccccc}
\centering
\tabletypesize{\tiny}
\tablenum{2}
%\topmargin 0.0cm \evensidemargin = 0mm
%\oddsidemargin=0mm \rotate \tabletypesize{\scriptsize}
\tablecaption{Continuum and emission-line parameters of the SDSS sample}
\tablehead{
\colhead{SDSS Name} &
\colhead{$z$} &
\colhead{$\log L_{5100}$} &
\colhead{FWHM(H$\beta^b$)} &
\colhead{$\log F$(H$\beta^{b}$)} &
\colhead{$\log F$(H$\beta^{n}$)} &
\colhead{$\log L_{3000}$} &
\colhead{FWHM(Mg\,II$^b$)} &
\colhead{$\log F$(Mg\,II$^b$)} &
\colhead{$\log F$(Mg\,II$^n$)} \\
\colhead{(1)}  & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)}
& \colhead{(6)} & \colhead{(7)}  & \colhead{(8)} & \colhead{(9)} & \colhead{(10)}
}
\startdata
    J000011.96$+$000225.3  &  0.478  &  44.69  &   3037  & -13.89  & -15.68  &  44.99  &   3284  & -13.84  & -14.89  \\
    J000110.97$-$105247.5  &  0.529  &  44.98  &   6807  & -13.73  & -15.53  &  45.18  &   5797  & -13.85  & -15.15  \\
    J001725.36$+$141132.6  &  0.514  &  45.23  &   5676  & -13.49  & -15.52  &  45.49  &   4432  & -13.64  & -14.71  \\
    J002019.22$-$110609.2  &  0.492  &  44.85  &   2832  & -13.74  & \nodata &  45.00  &   2677  & -13.91  & -16.16  \\
    J005121.25$+$004521.5  &  0.727  &  45.04  &   2572  & -14.09  & -15.07  &  45.14  &   1606  & -14.42  & -15.41  \\
    J005441.19$+$000110.7  &  0.646  &  45.08  &   2220  & -14.24  & \nodata &  45.13  &   2172  & -14.20  & -15.29  \\
    J010448.57$-$091013.0  &  0.469  &  44.77  &   4610  & -13.81  & -15.33  &  44.88  &   2627  & -14.11  & -15.86  \\
    J010644.16$-$103410.6  &  0.468  &  44.72  &   3873  & -13.83  & -15.35  &  44.85  &   3074  & -13.80  & -15.43  \\
    J011132.34$+$133519.0  &  0.576  &  45.13  &   8060  & -13.66  & -15.72  &  45.39  &   5495  & -13.73  & -14.87  \\
    J012016.73$-$092028.8  &  0.495  &  44.71  &   3284  & -13.72  & -16.02  &  45.05  &   3312  & -13.58  & -16.07  \\
    J014028.12$+$132320.7  &  0.493  &  44.84  &   2980  & -13.72  & -14.91  &  44.99  &   2431  & -13.92  & -15.15  \\
    J014247.75$-$084517.5  &  0.571  &  45.06  &   2550  & -14.02  & -14.87  &  45.22  &   2347  & -13.88  & -15.76  \\
    J014631.99$+$133506.3  &  0.688  &  45.33  &   3749  & -13.97  & -15.66  &  45.55  &   3993  & -13.72  & -15.39  \\
    J014718.41$-$082449.8  &  0.619  &  45.46  &   3139  & -13.48  & -15.18  &  45.69  &   2655  & -13.60  & \nodata \\
    J014942.51$+$001501.7  &  0.552  &  45.43  &   3640  & -13.30  & -15.18  &  45.70  &   3264  & -13.42  & -14.94  \\
    J015249.76$+$002314.7  &  0.589  &  44.98  &   1864  & -14.06  & \nodata &  45.10  &   2363  & -14.14  & -15.11  \\
    J015952.96$+$134554.4  &  0.503  &  44.72  &   2909  & -13.91  & -15.37  &  44.90  &   2431  & -14.01  & \nodata \\
    J020118.67$-$091935.8  &  0.661  &  45.08  &   3119  & -13.84  & -15.98  &  45.28  &   3610  & -13.93  & -14.92  \\
    J020413.09$-$090819.0  &  0.704  &  45.12  &   4877  & -13.80  & \nodata &  45.27  &   4437  & -14.16  & -15.30  \\
    J020435.19$-$093155.0  &  0.624  &  45.07  &   1883  & -14.06  & -16.97  &  45.23  &   1997  & -14.25  & -15.24  \\
    J024240.31$+$005727.2  &  0.569  &  45.50  &   3884  & -13.24  & -15.06  &  45.70  &   3937  & -13.27  & -14.23  \\
    J024651.91$-$005931.0  &  0.469  &  45.19  &   1898  & -13.52  & -15.02  &  45.34  &   2223  & -13.84  & -14.90  \\
    J024741.48$-$080240.7  &  0.569  &  44.96  &   9307  & -13.95  & \nodata &  45.21  &   6380  & -13.96  & \nodata \\
    J025508.24$-$081846.1  &  0.625  &  45.06  &   2025  & -13.95  & -15.92  &  45.22  &   2194  & -14.23  & -15.31  \\
    J025627.76$-$080134.9  &  0.474  &  44.84  &   2325  & -14.25  & -14.86  &  45.08  &   2050  & -14.17  & -15.42  \\
    J025937.47$+$003736.2  &  0.534  &  45.48  &   3356  & -13.36  & -15.09  &  45.68  &   3093  & -13.38  & -14.39  \\
    J030000.01$-$080357.0  &  0.561  &  45.45  &   2224  & -13.66  & -15.42  &  45.62  &   2919  & -13.61  & \nodata \\
    J030422.39$+$002231.8  &  0.642  &  45.63  &   3192  & -13.38  & -16.00  &  45.81  &   2623  & -13.62  & -16.29  \\
    J030911.64$+$002359.0  &  0.611  &  45.38  &   5528  & -13.47  & -14.99  &  45.71  &   3960  & -13.38  & -14.77  \\
    J032205.05$+$001201.5  &  0.471  &  44.98  &   4337  & -13.56  & -15.09  &  45.24  &   2979  & -13.59  & -15.34  \\
    J032205.05$+$001201.5  &  0.472  &  44.97  &   4068  & -13.59  & -15.47  &  45.23  &   3541  & -13.65  & -14.69  \\
    J033157.37$-$075549.7  &  0.526  &  44.91  &   3060  & -13.65  & -14.93  &  45.14  &   2787  & -13.69  & -15.22  \\
    J033438.28$-$071149.0  &  0.634  &  45.26  &   4740  & -13.59  & -16.11  &  45.50  &   3914  & -13.64  & -14.90  \\
    J035024.18$-$045315.5  &  0.715  &  45.39  &   2657  & -13.59  & -16.00  &  45.58  &   3388  & -13.63  & -14.58  \\
    J035118.00$+$001256.2  &  0.682  &  45.34  &   4764  & -13.67  & -16.31  &  45.58  &   3626  & -13.73  & -15.07  \\
    J035648.30$-$061238.6  &  0.711  &  45.15  &   4557  & -13.74  & -15.84  &  45.41  &   3274  & -13.96  & -15.15  \\
    J040148.98$-$054056.6  &  0.570  &  45.49  &   7634  & -13.49  & -16.33  &  45.58  &   5186  & -13.75  & -14.84  \\
    J040332.12$-$053713.9  &  0.631  &  44.91  &   6210  & -13.99  & -16.00  &  45.11  &   8103  & -13.95  & -14.99  \\
    J041204.52$-$045052.0  &  0.465  &  44.87  &   5980  & -14.04  & -15.83  &  44.96  &   3103  & -14.18  & -15.21  \\
    J041210.18$-$051109.3  &  0.549  &  45.23  &   4842  & -13.33  & -14.88  &  45.33  &   4238  & -13.66  & -15.29  \\
    J072307.86$+$420634.2  &  0.585  &  45.03  &   4192  & -13.79  & -15.41  &  45.26  &   4327  & -13.84  & -14.79  \\
    J073314.35$+$431049.0  &  0.500  &  44.89  &   2295  & -13.98  & -14.73  &  45.04  &   1165  & -14.07  & -15.02  \\
    J073356.03$+$410811.0  &  0.646  &  44.98  &   2888  & -13.83  & -15.41  &  45.23  &   2563  & -14.15  & -15.17  \\
    J073519.39$+$430918.1  &  0.629  &  45.12  &   3313  & -13.74  & -15.77  &  45.29  &   2365  & -14.04  & \nodata \\
    J073615.75$+$323026.5  &  0.569  &  44.65  &   2550  & -14.60  & -15.28  &  44.80  &   2375  & -14.49  & -15.58  \\
    J073722.18$+$241052.0  &  0.689  &  45.27  &   3684  & -13.81  & -15.21  &  45.43  &   2706  & -13.95  & -14.94  \\
    J073844.89$+$280153.5  &  0.720  &  45.18  &   3720  & -13.69  & \nodata &  45.49  &   3473  & -13.73  & \nodata \\
    J073912.65$+$400443.8  &  0.461  &  44.65  &   3747  & -13.95  & -15.20  &  44.85  &   3401  & -13.88  & -14.82  \\
    J073958.12$+$324223.0  &  0.563  &  44.87  &  12239  & -14.18  & -16.07  &  45.03  &   8356  & -14.07  & \nodata \\
    J074110.70$+$311200.2  &  0.632  &  45.50  &   4390  & -13.33  & \nodata &  45.71  &   3610  & -13.30  & -14.69  \\
    J074218.22$+$194719.5  &  0.658  &  45.27  &   7854  & -13.51  & -15.44  &  45.52  &   6973  & -13.46  & -15.12  \\
    J074541.67$+$314256.7  &  0.461  &  45.64  &   9976  & -12.83  & -14.56  &  45.81  &   5346  & -12.86  & -15.27  \\
    J074604.91$+$292250.3  &  0.547  &  44.89  &   4230  & -13.96  & -15.28  &  45.11  &   3185  & -14.04  & -15.86  \\
    J074619.19$+$444707.9  &  0.601  &  45.06  &   1592  & -13.90  & -16.02  &  45.15  &   1794  & -14.17  & -15.09  \\
    J074631.79$+$354523.7  &  0.600  &  44.87  &   1693  & -14.22  & -15.87  &  44.78  &   2132  & -14.52  & -15.56  \\
    J074642.60$+$360017.7  &  0.467  &  44.47  &   4787  & -14.23  & -16.14  &  44.62  &   3043  & -14.36  & -16.37  \\
    J074757.00$+$454527.7  &  0.726  &  45.47  &   4499  & -13.45  & -15.36  &  45.66  &   3301  & -13.71  & -14.90  \\
    J074840.53$+$154456.9  &  0.468  &  45.04  &   3652  & -13.68  & -15.46  &  45.18  &   3046  & -13.86  & -15.05  \\
    J074916.73$+$391307.8  &  0.464  &  44.91  &   3909  & -13.99  & -15.82  &  45.05  &   3791  & -13.98  & -15.21  \\
    J075101.87$+$335647.4  &  0.483  &  44.81  &   2282  & -13.85  & -15.67  &  44.92  &   2549  & -14.12  & -15.22  \\
    J075429.47$+$173450.3  &  0.572  &  44.95  &   5269  & -13.86  & -16.43  &  45.13  &   4450  & -13.91  & -15.57  \\
    J075515.07$+$185856.8  &  0.473  &  44.98  &   8060  & -13.72  & -15.74  &  45.16  &   4957  & -13.65  & -15.14  \\
    J080105.35$+$441041.1  &  0.471  &  45.09  &   7555  & -13.67  & -16.59  &  45.30  &   4541  & -13.82  & -14.92  \\
    J080216.97$+$294500.4  &  0.526  &  44.66  &   2371  & -14.11  & -15.90  &  44.81  &   2396  & -14.12  & -15.75  \\
    J080320.08$+$252602.4  &  0.477  &  44.78  &   3653  & -13.74  & -16.08  &  44.95  &   2494  & -14.02  & \nodata \\
    J080349.24$+$461010.0  &  0.515  &  44.85  &   4556  & -13.87  & -15.66  &  45.03  &   4077  & -13.84  & -15.67  \\
    J080642.14$+$425856.5  &  0.477  &  44.76  &   2787  & -13.93  & -15.64  &  44.85  &   1976  & -14.13  & -16.13  \\
    J080704.89$+$360353.6  &  0.468  &  44.82  &   3620  & -13.86  & -15.93  &  45.00  &   4054  & -14.03  & -15.20  \\
    J080742.13$+$412817.2  &  0.513  &  44.79  &   5098  & -13.96  & -15.52  &  44.98  &   3863  & -13.78  & -15.92  \\
    J080814.46$+$300914.8  &  0.540  &  44.78  &   3778  & -14.29  & -16.82  &  44.94  &   2430  & -14.27  & -15.17  \\
    J080814.70$+$475244.8  &  0.545  &  45.01  &   5677  & -13.74  & -15.58  &  45.12  &   7415  & -13.82  & -14.90  \\
    J080908.14$+$461925.6  &  0.659  &  45.64  &   3234  & -13.35  & -15.68  &  45.82  &   3672  & -13.57  & -14.60  \\
    J080945.43$+$293043.0  &  0.499  &  44.67  &   4994  & -14.07  & -16.06  &  44.86  &   3526  & -14.19  & \nodata \\
    J081100.60$+$571412.5  &  0.611  &  45.08  &   4572  & -13.65  & -15.57  &  45.31  &   4111  & -13.62  & -14.75  \\
    J081528.88$+$333254.3  &  0.482  &  44.69  &   4843  & -13.90  & -15.61  &  44.87  &   4328  & -13.84  & -15.25  \\
    J081558.07$+$501232.3  &  0.600  &  45.11  &   5200  & -13.61  & -16.19  &  45.24  &   3649  & -14.01  & -15.36  \\
    J082024.22$+$233450.5  &  0.470  &  44.91  &   2528  & -13.77  & -15.35  &  45.04  &   2415  & -13.82  & -31.15  \\
    J082045.37$+$243152.9  &  0.650  &  45.43  &   3056  & -13.57  & -15.32  &  45.71  &   2801  & -13.62  & -14.79  \\
    J082219.50$+$340044.9  &  0.726  &  45.27  &   4601  & -13.51  & -15.69  &  45.53  &   3689  & -13.45  & -14.99  \\
    J082329.16$+$473205.2  &  0.627  &  44.99  &   6282  & -13.84  & \nodata &  45.17  &   5246  & -13.91  & -15.86  \\
    J082439.00$+$405707.7  &  0.612  &  45.38  &   4828  & -13.51  & -14.90  &  45.50  &   2408  & -13.76  & -14.65  \\
    J082604.66$+$425435.8  &  0.710  &  45.16  &  10019  & -14.01  & -16.02  &  45.33  &   3612  & -14.01  & \nodata \\
    J082658.85$+$061142.7  &  0.495  &  44.94  &   2048  & -13.78  & -15.78  &  45.14  &   1497  & -14.15  & \nodata \\
    J082750.30$+$444847.6  &  0.530  &  44.62  &   4166  & -14.07  & \nodata &  44.83  &   3785  & -14.12  & \nodata \\
    J083010.51$+$321352.7  &  0.522  &  45.00  &   5206  & -13.77  & -15.03  &  45.22  &   4351  & -13.91  & -15.76  \\
    J083010.61$+$453321.4  &  0.668  &  44.85  &   7528  & -14.09  & -16.25  &  45.02  &   5783  & -14.26  & \nodata \\
    J083446.96$+$371656.5  &  0.574  &  45.11  &   2347  & -14.04  & -15.14  &  45.24  &   1876  & -14.16  & -15.25  \\
    J083510.37$+$035901.1  &  0.492  &  44.94  &   3989  & -13.62  & -15.76  &  45.20  &   3921  & -13.75  & -15.02  \\
    J083743.69$+$273419.3  &  0.697  &  45.29  &   4561  & -13.51  & -15.37  &  45.54  &   3630  & -13.67  & \nodata \\
    J084058.65$+$412520.6  &  0.693  &  45.28  &   3451  & -13.48  & -15.11  &  45.58  &   3382  & -13.51  & -14.78  \\
    J084252.54$+$342333.8  &  0.470  &  44.77  &   5338  & -13.70  & -16.31  &  45.14  &   4393  & -13.66  & -14.97  \\
    J084302.97$+$030218.9  &  0.511  &  45.61  &   2895  & -13.11  & -14.87  &  45.84  &   2500  & -13.41  & -14.38  \\
    J084437.98$+$412432.6  &  0.517  &  44.77  &   4701  & -13.92  & -15.84  &  44.95  &   3569  & -13.78  & -15.35  \\
    J084650.01$+$064149.0  &  0.617  &  45.21  &   8117  & -13.67  & -16.45  &  45.46  &   5038  & -13.64  & -15.44  \\
    J084650.01$+$064149.0  &  0.617  &  45.25  &   7864  & -13.56  & -16.39  &  45.41  &   5448  & -13.63  & -14.98  \\
    J084808.36$+$083208.2  &  0.712  &  45.35  &   2975  & -13.72  & -15.08  &  45.54  &   2034  & -14.00  & -16.00  \\
    J084818.85$+$025938.9  &  0.516  &  44.62  &   3911  & -14.07  & -15.83  &  44.75  &   3179  & -13.97  & \nodata \\
    J084902.61$+$300235.3  &  0.661  &  45.50  &   3715  & -13.25  & -15.22  &  45.69  &   3527  & -13.37  & -14.83  \\
    J084903.61$+$055905.9  &  0.533  &  44.80  &   5350  & -13.81  & -15.43  &  45.02  &   4357  & -13.90  & -14.96  \\
    J084959.49$+$431646.7  &  0.691  &  45.43  &   1993  & -13.91  & -15.04  &  45.56  &   2203  & -14.07  & -15.02  \\
    J085116.14$+$424328.9  &  0.482  &  44.81  &   4362  & -13.70  & -33.31  &  44.98  &   3628  & -13.85  & -16.45  \\
    J085217.18$+$434911.3  &  0.515  &  44.70  &   7039  & -13.81  & -15.65  &  44.89  &   5581  & -13.64  & -15.08  \\
    J085327.46$+$502938.2  &  0.496  &  44.82  &   4686  & -13.81  & -15.99  &  45.09  &   3401  & -14.04  & -15.52  \\
    J085334.25$+$434902.3  &  0.514  &  45.38  &   2621  & -13.30  & -14.91  &  45.57  &   2442  & -13.57  & -14.52  \\
    J085502.46$+$323918.4  &  0.617  &  45.09  &   3030  & -13.97  & -15.45  &  45.27  &   2243  & -14.09  & \nodata \\
    J085557.12$+$561534.7  &  0.714  &  45.51  &   2762  & -13.85  & -15.96  &  45.72  &   2972  & -13.80  & -14.89  \\
    J085559.00$+$005745.5  &  0.455  &  44.71  &   5301  & -13.88  & -16.36  &  44.90  &   4187  & -13.64  & -15.47  \\
    J085752.19$+$462152.8  &  0.554  &  45.02  &   5721  & -13.72  & -15.71  &  45.23  &   4203  & -13.66  & -15.16  \\
    J085830.61$+$080422.9  &  0.455  &  44.58  &   6621  & -13.95  & -15.22  &  44.79  &   5553  & -13.75  & \nodata \\
    J090007.99$+$364610.5  &  0.517  &  45.16  &  10615  & -13.58  & -15.14  &  45.40  &   8956  & -13.53  & -14.72  \\
    J090325.66$+$300525.1  &  0.538  &  44.74  &   7463  & -14.06  & -16.66  &  45.02  &   6205  & -13.98  & \nodata \\
    J090501.56$+$533907.5  &  0.594  &  44.96  &   6859  & -13.93  & -16.41  &  45.17  &   4290  & -13.88  & -14.83  \\
    J090743.67$+$551512.4  &  0.644  &  45.11  &   2814  & -13.89  & \nodata &  45.33  &   2983  & -13.95  & -15.34  \\
    J090745.29$+$532421.5  &  0.712  &  45.26  &   7185  & -13.97  & -16.06  &  45.46  &   7066  & -13.72  & -15.39  \\
    J090902.22$+$345926.5  &  0.575  &  45.01  &   7220  & -13.78  & -15.07  &  45.22  &   5561  & -13.68  & -15.23  \\
    J091029.76$+$101413.6  &  0.462  &  44.80  &   4154  & -13.84  & -17.32  &  45.06  &   3813  & -13.77  & -14.79  \\
    J091135.01$+$293803.8  &  0.614  &  45.05  &   2319  & -13.86  & -16.12  &  45.11  &   2307  & -14.01  & \nodata \\
    J091217.75$+$245037.9  &  0.652  &  45.75  &   4520  & -13.04  & -15.14  &  45.93  &   3697  & -13.24  & -15.39  \\
    J091257.08$+$275646.7  &  0.513  &  44.97  &   3545  & -13.84  & -15.61  &  45.15  &   2456  & -13.99  & -15.92  \\
    J091327.14$+$011149.0  &  0.551  &  44.98  &   5889  & -14.13  & \nodata &  45.07  &   2854  & -14.17  & -16.24  \\
    J091431.78$+$083742.8  &  0.649  &  45.40  &   3645  & -13.53  & -15.47  &  45.58  &   3203  & -13.80  & -15.30  \\
    J091451.42$+$421956.9  &  0.549  &  44.99  &   2729  & -13.77  & -14.64  &  45.19  &   1940  & -13.97  & -14.92  \\
    J091501.64$+$081248.7  &  0.507  &  44.67  &   6913  & -13.95  & -15.87  &  44.90  &   5036  & -13.98  & -15.21  \\
    J091616.00$+$392657.3  &  0.533  &  44.85  &   8224  & -13.71  & -15.40  &  45.03  &   6780  & -13.56  & -14.94  \\
    J091625.40$+$471441.6  &  0.538  &  45.33  &   2844  & -13.43  & -15.50  &  45.50  &   2334  & -13.69  & -14.62  \\
    J091741.63$+$034012.9  &  0.536  &  44.89  &   4266  & -13.84  & \nodata &  45.17  &   3906  & -13.94  & -14.96  \\
    J091957.60$+$510609.6  &  0.554  &  45.48  &   4272  & -13.26  & -16.02  &  45.71  &   3870  & -13.48  & -14.79  \\
    J092020.79$+$280034.7  &  0.558  &  44.98  &   2490  & -14.01  & -15.26  &  45.04  &   2630  & -14.14  & -15.27  \\
    J092133.02$+$321320.5  &  0.585  &  45.33  &   6746  & -13.58  & -15.34  &  45.48  &   4321  & -13.81  & -14.75  \\
    J092223.08$+$062753.8  &  0.519  &  44.94  &   4656  & -13.89  & \nodata &  45.12  &   3687  & -13.91  & -15.01  \\
    J092317.15$+$011352.5  &  0.595  &  44.94  &   1849  & -14.06  & -15.39  &  45.10  &   2069  & -14.12  & -15.02  \\
    J092358.79$+$584906.2  &  0.709  &  45.59  &   2896  & -13.37  & -15.36  &  45.83  &   2695  & -13.63  & -14.57  \\
    J092415.68$+$102824.6  &  0.511  &  44.70  &   4711  & -14.17  & -15.74  &  44.93  &   2644  & -14.21  & -16.07  \\
    J092423.43$+$064250.7  &  0.589  &  45.25  &   4092  & -13.49  & -15.46  &  45.46  &   3582  & -13.66  & -14.93  \\
    J092441.08$-$001729.6  &  0.707  &  45.15  &   4494  & -13.86  & -15.58  &  45.23  &   3521  & -14.12  & -15.02  \\
    J092514.37$+$544427.1  &  0.474  &  45.32  &   5844  & -13.15  & -14.92  &  45.52  &   5068  & -13.22  & -14.45  \\
    J092554.71$+$400414.1  &  0.471  &  44.99  &   9170  & -13.68  & -15.78  &  45.17  &   7250  & -13.67  & -15.16  \\
    J092646.58$+$281206.6  &  0.484  &  44.70  &   9377  & -13.92  & -16.20  &  45.03  &   5954  & -13.72  & -15.39  \\
    J092703.02$+$390220.9  &  0.695  &  45.52  &   5300  & -13.47  & -15.19  &  45.74  &   4002  & -13.36  & -16.52  \\
    J092703.20$+$522316.5  &  0.602  &  45.43  &   4824  & -13.48  & -15.43  &  45.64  &   4493  & -13.78  & -14.78  \\
    J092809.43$+$383000.6  &  0.498  &  45.29  &   5845  & -13.49  & \nodata &  45.44  &   2800  & -13.56  & -16.05  \\
    J092820.80$+$390446.4  &  0.666  &  45.50  &   3107  & -13.63  & -14.61  &  45.63  &   2378  & -13.76  & -14.77  \\
    J092943.42$+$004127.4  &  0.587  &  45.37  &   2164  & -13.55  & -14.38  &  45.54  &   1968  & -13.80  & -14.71  \\
    J093211.69$+$315709.7  &  0.537  &  44.86  &   3196  & -13.83  & -15.96  &  45.09  &   3896  & -13.90  & -14.85  \\
    J093255.46$+$284036.8  &  0.547  &  45.26  &   6738  & -13.39  & -15.23  &  45.44  &   6463  & -13.12  & -14.65  \\
    J093457.84$+$343129.8  &  0.514  &  44.71  &   3478  & -13.86  & -15.79  &  44.94  &   3327  & -14.01  & -15.51  \\
    J093502.54$+$433110.7  &  0.458  &  45.46  &   8277  & -13.05  & -15.50  &  45.69  &   4296  & -13.03  & \nodata \\
    J093518.19$+$020415.5  &  0.650  &  45.25  &   8179  & -13.49  & \nodata &  45.48  &   7415  & -13.34  & -14.82  \\
    J093642.97$+$551119.4  &  0.498  &  44.54  &  12215  & -14.36  & -15.92  &  44.63  &   9704  & -14.06  & \nodata \\
    J093704.04$+$293704.8  &  0.451  &  44.79  &   5569  & -13.86  & -16.18  &  44.99  &   4047  & -14.10  & -15.98  \\
    J093732.81$+$543707.8  &  0.469  &  44.97  &   4449  & -13.47  & -15.60  &  45.16  &   3859  & -13.54  & -14.80  \\
    J093814.17$+$284402.3  &  0.524  &  44.81  &   3365  & -14.01  & -16.14  &  45.04  &   3710  & -14.26  & -15.28  \\
    J093857.99$+$614019.7  &  0.736  &  45.31  &   4926  & -13.64  & -15.78  &  45.50  &   3639  & -13.82  & -16.06  \\
    J093911.25$+$100712.4  &  0.663  &  45.11  &   3490  & -13.86  & -15.87  &  45.34  &   3306  & -14.03  & -15.39  \\
    J093930.10$+$514103.6  &  0.605  &  45.02  &   2369  & -13.98  & -14.80  &  45.28  &   2061  & -14.15  & -15.04  \\
    J093944.54$+$392402.8  &  0.455  &  45.09  &   2943  & -13.50  & -15.32  &  45.39  &   2207  & -13.53  & -14.43  \\
    J094033.76$+$462315.0  &  0.697  &  45.34  &   1903  & -13.69  & -16.08  &  45.49  &   2214  & -14.11  & -15.18  \\
    J094324.33$+$283540.3  &  0.460  &  44.69  &   2067  & -14.23  & -14.99  &  44.82  &   1940  & -14.21  & -15.29  \\
    J094331.62$+$053131.5  &  0.564  &  45.29  &   2471  & -13.67  & -14.75  &  45.46  &   1845  & -13.90  & -14.86  \\
    J094430.78$+$435421.4  &  0.587  &  44.98  &  10422  & -13.79  & -15.68  &  45.16  &   5775  & -13.99  & -16.12  \\
    J094443.09$+$580953.2  &  0.562  &  44.89  &   7145  & -13.93  & -34.19  &  45.04  &   5622  & -13.73  & \nodata \\
    J094549.25$+$344545.9  &  0.507  &  44.68  &   2680  & -14.02  & -16.20  &  44.93  &   2737  & -14.01  & \nodata \\
    J094712.66$+$530612.9  &  0.480  &  44.53  &   2390  & -14.03  & -15.46  &  44.83  &   2735  & -13.95  & -16.10  \\
    J094715.56$+$631716.5  &  0.488  &  45.38  &   6168  & -13.12  & -15.41  &  45.56  &   4206  & -13.16  & -14.76  \\
    J094756.00$+$535000.4  &  0.483  &  45.11  &   4926  & -13.23  & -14.43  &  45.35  &   3271  & -13.40  & -14.38  \\
    J094945.69$+$632622.9  &  0.650  &  45.03  &   2331  & -14.01  & -16.31  &  45.20  &   2130  & -14.14  & -16.20  \\
    J095000.74$+$483129.3  &  0.589  &  45.18  &   3145  & -13.60  & -15.44  &  45.39  &   2914  & -13.88  & -14.83  \\
    J095257.15$+$050910.3  &  0.543  &  45.17  &   2769  & -13.70  & -14.72  &  45.40  &   2031  & -13.84  & -14.82  \\
    J095524.74$+$284629.1  &  0.549  &  45.12  &   1959  & -13.71  & -15.83  &  45.28  &   2267  & -13.86  & -14.87  \\
    J095528.39$+$435734.5  &  0.464  &  44.96  &   6971  & -13.79  & -18.35  &  45.04  &   4007  & -13.84  & -14.81  \\
    J095623.21$+$323621.7  &  0.526  &  44.96  &   2860  & -13.82  & -15.48  &  45.19  &   2532  & -13.87  & -14.78  \\
    J095650.14$+$515212.2  &  0.676  &  45.29  &   1790  & -13.87  & -15.79  &  45.36  &   1890  & -14.06  & -15.57  \\
    J095702.82$+$563136.0  &  0.689  &  45.15  &   4035  & -13.73  & -15.84  &  45.37  &   3953  & -14.09  & -15.01  \\
    J095758.45$-$002354.1  &  0.595  &  45.32  &   4853  & -13.41  & \nodata &  45.54  &   4138  & -13.64  & -16.04  \\
    J095830.61$+$392354.4  &  0.489  &  45.08  &   4248  & -13.73  & -15.26  &  45.17  &   3204  & -14.24  & -15.38  \\
    J095851.80$+$123755.3  &  0.599  &  45.20  &   3925  & -13.52  & -17.50  &  45.43  &   3528  & -13.74  & -14.91  \\
    J095914.85$+$320357.3  &  0.564  &  45.21  &   8049  & -13.51  & \nodata &  45.44  &   5638  & -13.59  & -15.38  \\
    J095930.54$+$300734.4  &  0.544  &  44.86  &  10603  & -13.83  & -15.93  &  45.15  &   9931  & -13.87  & -15.09  \\
    J100056.54$+$011319.1  &  0.520  &  44.78  &   1921  & -14.13  & -15.62  &  44.83  &   2242  & -14.41  & -15.43  \\
    J100102.57$+$594414.4  &  0.747  &  45.87  &   3265  & -13.27  & -14.62  &  46.09  &   2450  & -13.61  & -14.85  \\
    J100226.55$+$342756.8  &  0.689  &  45.15  &   4107  & -13.74  & -15.49  &  45.36  &   3005  & -13.97  & -15.20  \\
    J100324.57$+$021831.3  &  0.518  &  44.67  &   4162  & -14.14  & -16.01  &  44.86  &   3051  & -14.17  & -15.55  \\
    J100721.79$+$611541.4  &  0.702  &  45.21  &   5773  & -13.72  & -15.86  &  45.48  &   4066  & -13.88  & -15.17  \\
    J100902.07$+$071343.9  &  0.456  &  45.13  &   8392  & -13.51  & -15.54  &  45.30  &   5689  & -13.55  & \nodata \\
    J101027.52$+$413239.1  &  0.612  &  45.53  &   3521  & -13.28  & -15.52  &  45.82  &   4037  & -13.24  & -14.17  \\
    J101107.76$+$035750.6  &  0.593  &  44.91  &   9117  & -14.01  & -17.53  &  45.08  &   5982  & -14.04  & -16.29  \\
    J101424.84$+$084314.1  &  0.625  &  45.21  &   3719  & -13.94  & \nodata &  45.42  &   3327  & -14.00  & -15.52  \\
    J101636.42$+$124959.7  &  0.469  &  44.75  &   2918  & -13.71  & -15.14  &  44.95  &   2592  & -13.85  & -14.87  \\
    J102056.37$+$100332.8  &  0.608  &  45.06  &   4211  & -13.89  & \nodata &  45.30  &   3702  & -13.85  & -16.05  \\
    J102237.45$+$393150.2  &  0.603  &  45.33  &   5416  & -14.34  & -15.57  &  45.30  &   4244  & -13.74  & -15.55  \\
    J102322.27$+$363912.4  &  0.545  &  44.84  &   4019  & -14.13  & \nodata &  44.92  &   2646  & -14.08  & -15.20  \\
    J102750.58$+$073315.7  &  0.587  &  45.08  &   5377  & -13.52  & -15.73  &  45.31  &   5185  & -13.45  & -14.83  \\
    J102832.78$+$650247.8  &  0.552  &  44.83  &   7321  & -13.91  & -15.35  &  45.00  &   7753  & -13.97  & -14.97  \\
    J102838.76$+$111823.2  &  0.504  &  44.85  &   3108  & -13.80  & -15.02  &  45.01  &   2521  & -13.82  & \nodata \\
    J102847.01$+$391800.5  &  0.473  &  44.95  &   3630  & -13.53  & -15.57  &  45.26  &   3269  & -13.52  & -14.75  \\
    J102950.71$+$471110.1  &  0.521  &  44.98  &   4034  & -13.78  & -15.28  &  45.20  &   2950  & -13.91  & -31.13  \\
    J103105.96$+$084743.7  &  0.635  &  45.16  &   3414  & -13.73  & \nodata &  45.40  &   2876  & -13.93  & -16.06  \\
    J103205.45$+$114946.8  &  0.725  &  45.42  &   3665  & -13.94  & \nodata &  45.51  &   2946  & -13.92  & -16.34  \\
    J103440.92$+$443105.0  &  0.534  &  45.08  &   5680  & -13.80  & -15.58  &  45.32  &   4216  & -13.69  & -15.03  \\
    J103539.87$+$663430.4  &  0.454  &  44.91  &   5212  & -13.56  & -15.31  &  45.14  &   4203  & -13.77  & -14.89  \\
    J104011.19$+$452126.0  &  0.546  &  45.01  &   2816  & -14.23  & -15.18  &  45.13  &   2607  & -14.18  & \nodata \\
    J104013.48$+$383544.4  &  0.534  &  45.21  &   5316  & -13.38  & -15.47  &  45.34  &   4448  & -13.64  & -15.54  \\
    J104122.84$-$005618.5  &  0.497  &  44.62  &   4181  & -14.09  & -15.63  &  44.79  &   3019  & -14.06  & -15.37  \\
    J104146.77$+$523328.2  &  0.678  &  45.49  &   4111  & -13.45  & -15.68  &  45.74  &   3641  & -13.44  & -14.78  \\
    J104218.33$+$501243.9  &  0.470  &  44.85  &   4249  & -13.80  & -15.81  &  45.07  &   3034  & -13.99  & -16.05  \\
    J104431.77$+$070841.1  &  0.646  &  45.28  &   2023  & -14.09  & \nodata &  45.43  &   2634  & -14.14  & -15.57  \\
    J104529.74$+$013350.6  &  0.688  &  45.20  &   2106  & -13.76  & -15.53  &  45.41  &   1918  & -14.02  & -15.14  \\
    J104545.69$+$430842.0  &  0.653  &  45.27  &   3923  & -13.73  & -15.57  &  45.38  &   2802  & -13.92  & \nodata \\
    J104613.74$+$525554.2  &  0.504  &  45.02  &   2151  & -14.17  & -15.10  &  45.22  &   3080  & -14.20  & -15.25  \\
    J104708.08$+$144557.8  &  0.705  &  45.19  &   5538  & -14.28  & -15.71  &  45.28  &   6153  & -14.30  & -15.54  \\
    J104831.21$+$393147.1  &  0.543  &  44.96  &   1967  & -13.86  & -15.33  &  45.19  &   2035  & -13.97  & -14.94  \\
    J104924.72$+$142627.9  &  0.573  &  44.88  &   4851  & -13.88  & -15.62  &  45.09  &   4690  & -13.92  & -14.89  \\
    J105122.29$+$020736.6  &  0.599  &  45.18  &   3045  & -13.47  & -15.42  &  45.40  &   2927  & -13.70  & -15.25  \\
    J105157.24$+$375429.1  &  0.562  &  45.09  &   6170  & -13.64  & -16.73  &  45.32  &   4708  & -13.70  & -15.35  \\
    J105205.58$+$364039.7  &  0.608  &  45.36  &   2811  & -13.72  & -14.86  &  45.56  &   2989  & -13.78  & -14.88  \\
    J105540.81$+$421241.2  &  0.636  &  44.94  &   3479  & -13.91  & -16.22  &  45.16  &   2415  & -14.15  & \nodata \\
    J105600.08$+$142411.4  &  0.623  &  45.22  &   2107  & -13.93  & -16.22  &  45.38  &   3114  & -14.02  & -15.21  \\
    J105742.11$+$651814.4  &  0.523  &  44.72  &   5747  & -14.00  & \nodata &  44.88  &   4188  & -14.30  & -15.34  \\
    J105945.23$+$144143.0  &  0.631  &  45.35  &   5120  & -13.44  & -15.50  &  45.53  &   4386  & -13.70  & -14.89  \\
    J110046.80$+$345502.7  &  0.591  &  45.10  &   2521  & -13.72  & -15.37  &  45.31  &   2133  & -14.14  & -15.02  \\
    J110236.66$+$052117.1  &  0.499  &  44.82  &   2755  & -13.80  & -15.77  &  45.00  &   2911  & -13.94  & -15.17  \\
    J110246.15$+$314513.1  &  0.531  &  44.77  &   2607  & -13.88  & -15.83  &  45.01  &   2486  & -14.09  & -15.00  \\
    J110409.63$+$122157.5  &  0.591  &  45.07  &   5493  & -13.75  & -32.38  &  45.32  &   4593  & -13.62  & -14.83  \\
    J110535.67$+$310804.6  &  0.552  &  44.98  &   4968  & -13.68  & -16.05  &  45.21  &   6415  & -13.83  & -14.78  \\
    J110539.82$+$342534.6  &  0.506  &  45.55  &   3785  & -13.10  & -15.82  &  45.74  &   3078  & -13.27  & -14.75  \\
    J110631.06$+$351051.3  &  0.485  &  44.77  &   2233  & -13.90  & -15.94  &  44.95  &   2845  & -13.97  & -14.97  \\
    J110651.78$+$135527.0  &  0.566  &  44.91  &   4456  & -14.30  & -16.13  &  44.96  &   4411  & -14.29  & -15.27  \\
    J110705.75$+$105746.4  &  0.565  &  45.11  &   2856  & -13.72  & -15.26  &  45.30  &   2892  & -13.91  & -14.83  \\
    J110913.61$+$044503.1  &  0.637  &  44.96  &   7840  & -13.91  & -15.61  &  45.04  &   4712  & -13.88  & -15.77  \\
    J111123.80$+$505131.1  &  0.559  &  44.90  &   2846  & -14.07  & -14.98  &  45.04  &   2124  & -14.15  & -15.10  \\
    J111239.11$+$353928.2  &  0.636  &  45.07  &   5700  & -13.72  & -15.54  &  45.34  &   5401  & -13.85  & -14.87  \\
    J111320.62$+$641053.5  &  0.572  &  45.17  &   5822  & -13.68  & -16.38  &  45.34  &   4449  & -13.73  & -15.13  \\
    J111458.11$+$511738.5  &  0.665  &  45.30  &   5740  & -13.57  & -15.05  &  45.49  &   3416  & -13.76  & -15.36  \\
    J111507.66$+$023757.6  &  0.567  &  45.17  &   2865  & -13.54  & -15.75  &  45.37  &   2882  & -13.78  & -14.81  \\
    J111909.52$+$153216.4  &  0.674  &  45.41  &   2376  & -13.91  & -15.36  &  45.48  &   3706  & -13.89  & -14.99  \\
    J111941.14$+$595108.7  &  0.488  &  44.95  &   1979  & -13.89  & -14.87  &  45.10  &   1646  & -14.15  & -15.51  \\
    J112005.00$+$041323.3  &  0.545  &  45.13  &   2886  & -13.64  & -15.21  &  45.27  &   2402  & -13.84  & \nodata \\
    J112021.13$+$404517.3  &  0.584  &  45.31  &   3426  & -13.56  & -15.43  &  45.48  &   2743  & -13.98  & -14.94  \\
    J112119.91$+$004308.0  &  0.546  &  44.88  &   4733  & -13.98  & -15.51  &  44.99  &   3727  & -14.10  & -15.03  \\
    J112158.37$+$651716.2  &  0.501  &  45.12  &   2953  & -13.47  & \nodata &  45.28  &   2852  & -13.99  & -15.05  \\
    J112224.16$+$031802.6  &  0.475  &  44.94  &   3313  & -13.82  & -16.35  &  45.05  &   2547  & -14.04  & -15.16  \\
    J112448.29$+$531818.8  &  0.531  &  44.83  &   3422  & -13.91  & -15.59  &  45.07  &   2877  & -13.94  & -31.13  \\
    J112621.31$+$314416.4  &  0.480  &  44.61  &   5066  & -14.12  & -15.89  &  44.80  &   3439  & -14.30  & \nodata \\
    J112707.67$+$035825.0  &  0.544  &  45.08  &   3381  & -13.63  & -15.46  &  45.32  &   3146  & -13.64  & \nodata \\
    J112755.55$+$103839.9  &  0.635  &  45.22  &   4028  & -14.13  & \nodata &  45.44  &   4128  & -14.10  & -15.17  \\
    J112756.77$+$115427.1  &  0.506  &  45.13  &   2167  & -13.57  & \nodata &  45.28  &   3244  & -13.66  & -14.70  \\
    J112757.42$+$644118.4  &  0.694  &  45.28  &   1721  & -13.86  & -32.95  &  45.41  &   2418  & -13.99  & -15.03  \\
    J113046.17$+$072250.2  &  0.493  &  45.01  &   6476  & -13.57  & -15.54  &  45.23  &   5326  & -13.72  & -14.76  \\
    J113259.49$+$102342.2  &  0.539  &  45.17  &   2737  & -13.51  & -15.11  &  45.40  &   2875  & -13.72  & -15.08  \\
    J113327.79$+$032719.4  &  0.524  &  44.93  &   3090  & -13.83  & -15.33  &  45.07  &   3127  & -13.78  & -14.71  \\
    J113330.30$+$105223.3  &  0.511  &  45.51  &  14199  & -13.17  & -15.03  &  45.74  &   7578  & -13.15  & -15.14  \\
    J113401.98$+$060640.6  &  0.574  &  45.06  &   6833  & -14.20  & -15.99  &  45.21  &   5091  & -13.92  & -15.23  \\
    J113411.53$+$645107.3  &  0.614  &  45.26  &   3077  & -13.42  & -15.39  &  45.46  &   2554  & -13.81  & -14.73  \\
    J113615.14$+$103430.9  &  0.523  &  45.39  &   3274  & -13.26  & -14.87  &  45.61  &   3008  & -13.37  & -14.97  \\
    J113635.95$+$063113.7  &  0.528  &  45.17  &   5553  & -13.45  & -15.59  &  45.43  &   4328  & -13.53  & -14.73  \\
    J113801.84$+$490506.5  &  0.480  &  44.82  &   6500  & -13.77  & -16.05  &  44.96  &   5411  & -13.92  & -15.23  \\
    J113909.24$+$035432.5  &  0.550  &  44.90  &   4480  & -13.83  & \nodata &  45.11  &   4024  & -13.80  & -15.93  \\
    J113944.64$+$121436.1  &  0.618  &  45.07  &   2150  & -13.87  & \nodata &  45.23  &   2074  & -14.18  & \nodata \\
    J114106.46$+$513237.7  &  0.539  &  44.92  &   6910  & -13.81  & -15.71  &  45.15  &   5824  & -13.82  & -15.29  \\
    J114117.63$-$001250.4  &  0.504  &  44.87  &   8590  & -14.02  & -15.97  &  45.13  &   6824  & -13.77  & -15.89  \\
    J114125.81$+$070652.4  &  0.498  &  44.92  &   2134  & -14.04  & -16.11  &  45.01  &   2314  & -14.19  & -15.11  \\
    J114315.76$+$111351.8  &  0.565  &  44.97  &   2171  & -13.72  & -15.70  &  45.19  &   2277  & -13.94  & -15.83  \\
    J114435.63$+$463757.5  &  0.662  &  45.31  &   2787  & -13.82  & -14.63  &  45.43  &   1821  & -14.12  & -15.14  \\
    J114541.67$+$671227.6  &  0.514  &  44.65  &   2162  & -14.12  & -15.70  &  44.94  &   2017  & -14.32  & -15.30  \\
    J114552.19$+$620633.7  &  0.749  &  45.41  &   3253  & -13.70  & -16.13  &  45.66  &   2999  & -13.92  & -15.08  \\
    J114805.31$-$023303.6  &  0.566  &  45.02  &   2270  & -13.83  & -14.98  &  45.20  &   1889  & -14.01  & -16.11  \\
    J114818.88$+$315410.1  &  0.550  &  45.04  &   2883  & -13.65  & -15.86  &  45.33  &   3023  & -13.77  & -14.69  \\
    J114913.93$-$014454.0  &  0.458  &  45.16  &   3268  & -13.33  & -15.10  &  45.39  &   3167  & -13.51  & -14.48  \\
    J115026.53$+$015928.0  &  0.581  &  44.96  &   4807  & -13.98  & -15.65  &  45.14  &   3549  & -13.92  & -15.66  \\
    J115050.82$+$110726.0  &  0.692  &  45.30  &   4415  & -13.70  & -15.52  &  45.45  &   3356  & -13.91  & -14.85  \\
    J115315.02$+$320223.9  &  0.590  &  44.98  &   2355  & -13.88  & -15.46  &  45.16  &   2488  & -13.99  & -16.01  \\
    J115412.07$+$463552.2  &  0.642  &  45.20  &   7029  & -13.62  & -15.60  &  45.42  &   5138  & -13.54  & -14.73  \\
    J115426.58$+$583153.5  &  0.703  &  45.42  &   5875  & -13.63  & -15.47  &  45.45  &   4353  & -13.86  & -14.79  \\
    J115554.41$+$445628.3  &  0.521  &  45.00  &   7744  & -13.59  & -15.54  &  45.18  &   5605  & -13.48  & -15.10  \\
    J115651.66$+$115636.2  &  0.645  &  45.48  &  11022  & -13.35  & -15.46  &  45.70  &   5434  & -13.59  & -15.83  \\
    J115741.43$+$151414.1  &  0.750  &  45.65  &   3293  & -13.64  & -15.77  &  45.78  &   2449  & -13.94  & -15.45  \\
    J115839.92$+$625427.9  &  0.592  &  45.57  &  11779  & -13.15  & -15.03  &  45.73  &  10714  & -13.45  & -14.56  \\
    J115906.79$+$530643.3  &  0.482  &  44.95  &   2978  & -13.56  & -15.42  &  45.12  &   2376  & -13.85  & -14.83  \\
    J120402.86$+$565920.9  &  0.576  &  44.76  &   3185  & -13.82  & -15.67  &  45.04  &   3107  & -13.98  & -14.89  \\
    J120407.58$+$341916.3  &  0.522  &  44.84  &   8230  & -13.89  & -16.30  &  45.02  &   6502  & -14.01  & -16.23  \\
    J120422.33$+$380836.9  &  0.566  &  45.10  &   3557  & -13.54  & -16.29  &  45.31  &   2804  & -13.66  & -15.94  \\
    J120424.03$+$433056.9  &  0.662  &  45.68  &  12420  & -13.14  & -16.19  &  45.92  &   6638  & -13.26  & -15.60  \\
    J120436.17$+$485653.9  &  0.451  &  44.60  &   3421  & -14.02  & -15.44  &  44.73  &   2871  & -13.86  & -16.05  \\
    J120436.17$+$485653.9  &  0.451  &  44.69  &   3518  & -13.92  & -15.29  &  44.88  &   2658  & -13.79  & \nodata \\
    J120633.08$+$412536.1  &  0.554  &  45.24  &   1898  & -13.89  & -15.28  &  45.20  &   2950  & -13.93  & -15.61  \\
    J121144.43$+$361156.9  &  0.561  &  44.92  &   5056  & -13.74  & -32.69  &  45.13  &   3919  & -13.87  & -14.99  \\
    J121248.05$+$615340.5  &  0.608  &  45.29  &   4321  & -13.47  & -15.77  &  45.51  &   3486  & -13.52  & -15.52  \\
    J121430.55$+$082508.2  &  0.586  &  45.23  &  10121  & -13.50  & -15.09  &  45.42  &   7941  & -13.49  & -14.73  \\
    J121509.22$+$330955.2  &  0.615  &  45.52  &   5017  & -13.24  & -15.36  &  45.76  &   4097  & -13.21  & -14.66  \\
    J121640.57$+$071224.3  &  0.587  &  45.30  &   8146  & -13.56  & -15.95  &  45.54  &   5931  & -13.49  & -15.41  \\
    J121707.71$+$604850.5  &  0.693  &  45.43  &   2706  & -13.69  & -15.90  &  45.64  &   2447  & -13.75  & -14.75  \\
    J121708.55$+$662447.5  &  0.585  &  45.25  &   9898  & -13.61  & \nodata &  45.52  &   5376  & -13.52  & -15.35  \\
    J121740.81$+$493118.1  &  0.732  &  45.40  &   5299  & -13.55  & -15.65  &  45.53  &   4424  & -13.61  & -14.56  \\
    J121850.52$+$101554.2  &  0.541  &  45.09  &   2336  & -14.07  & -14.93  &  45.24  &   2528  & -13.93  & -15.17  \\
    J122106.87$+$454852.1  &  0.525  &  45.06  &   4975  & -13.57  & -15.89  &  45.31  &   4597  & -13.65  & -14.63  \\
    J122233.53$+$382754.3  &  0.532  &  44.79  &   8614  & -13.60  & \nodata &  45.06  &   7897  & -13.53  & \nodata \\
    J122520.13$+$084450.8  &  0.535  &  45.06  &   3897  & -13.85  & -15.49  &  45.26  &   3424  & -13.75  & \nodata \\
    J122557.86$+$364907.7  &  0.476  &  44.99  &   3306  & -13.69  & -15.05  &  45.14  &   2317  & -13.85  & -15.79  \\
    J122924.15$+$410509.6  &  0.685  &  45.28  &   4515  & -13.68  & \nodata &  45.53  &   3671  & -13.83  & -16.27  \\
    J123046.35$+$650607.0  &  0.477  &  44.88  &   3193  & -13.85  & -15.97  &  45.02  &   2607  & -14.01  & -15.51  \\
    J123304.06$-$003134.1  &  0.470  &  44.88  &   3290  & -14.08  & -15.62  &  45.09  &   3279  & -14.18  & -15.56  \\
    J123516.14$+$462309.5  &  0.544  &  45.12  &   4361  & -13.88  & -16.67  &  45.27  &   3534  & -13.81  & -14.82  \\
    J123734.47$+$444731.7  &  0.461  &  44.94  &   4333  & -13.79  & -15.13  &  45.13  &   3894  & -14.02  & -15.02  \\
    J123915.93$+$084639.4  &  0.506  &  45.01  &   3158  & -13.70  & -15.46  &  45.15  &   3011  & -13.99  & -14.93  \\
    J124139.73$+$493405.5  &  0.474  &  44.89  &   8068  & -13.75  & -15.71  &  45.04  &   6779  & -13.89  & -15.22  \\
    J124307.86$+$345943.0  &  0.537  &  44.94  &   6618  & -13.76  & -15.90  &  45.20  &   6108  & -13.72  & -14.82  \\
    J124335.42$+$421520.6  &  0.511  &  44.89  &   4545  & -13.77  & -15.59  &  45.12  &   3369  & -13.71  & -15.23  \\
    J124354.67$+$371823.9  &  0.592  &  45.04  &   6504  & -13.65  & -15.53  &  45.19  &   9342  & -13.62  & -14.86  \\
    J124456.24$-$013933.7  &  0.492  &  44.85  &   5850  & -13.64  & -15.24  &  45.08  &   4874  & -13.75  & -14.88  \\
    J124503.56$+$422844.0  &  0.478  &  44.74  &   8135  & -13.87  & -15.70  &  44.95  &   5495  & -14.06  & -15.65  \\
    J124537.49$+$144857.4  &  0.554  &  45.12  &   2340  & -13.83  & -15.24  &  45.27  &   2226  & -14.05  & -14.96  \\
    J124613.13$-$004233.0  &  0.649  &  45.38  &   2532  & -13.63  & -15.96  &  45.66  &   3092  & -13.69  & \nodata \\
    J124654.03$+$131310.7  &  0.512  &  45.37  &   3150  & -13.40  & -14.56  &  45.57  &   2178  & -13.66  & -15.06  \\
    J124705.53$+$395737.7  &  0.455  &  44.71  &   6002  & -13.93  & -15.85  &  44.85  &   4656  & -14.10  & -15.09  \\
    J124905.48$+$475825.4  &  0.617  &  45.23  &   6077  & -13.72  & -15.49  &  45.45  &   3856  & -13.78  & -15.63  \\
    J125304.51$+$024704.3  &  0.538  &  44.88  &   3040  & -13.78  & -15.49  &  45.14  &   3371  & -13.84  & -14.79  \\
    J125415.56$+$480850.7  &  0.503  &  44.84  &   3575  & -13.65  & \nodata &  45.06  &   3417  & -13.82  & -15.36  \\
    J125436.41$+$053720.4  &  0.512  &  45.14  &   4516  & -13.43  & -15.35  &  45.35  &   5031  & -13.24  & -14.35  \\
    J125457.82$+$033644.6  &  0.487  &  44.72  &   5150  & -13.99  & \nodata &  44.89  &   4572  & -13.78  & -15.23  \\
    J125901.68$+$413055.8  &  0.745  &  45.61  &   5667  & -13.42  & -15.47  &  45.76  &   4251  & -13.89  & -14.83  \\
    J130028.54$+$283010.2  &  0.647  &  45.34  &  10336  & -13.55  & -15.50  &  45.56  &   8443  & -13.53  & \nodata \\
    J130112.93$+$590206.8  &  0.476  &  45.62  &   2933  & -13.19  & -14.68  &  45.89  &   2883  & -13.37  & -14.56  \\
    J130139.77$+$545930.5  &  0.462  &  44.94  &   2440  & -13.76  & -15.56  &  45.03  &   2524  & -14.06  & -15.00  \\
    J130524.26$+$035731.0  &  0.545  &  44.99  &   6986  & -13.74  & -16.61  &  45.24  &   5424  & -13.61  & \nodata \\
    J130543.82$+$333531.6  &  0.488  &  44.80  &   3859  & -13.80  & -15.64  &  44.99  &   3136  & -13.87  & \nodata \\
    J130832.10$+$034404.0  &  0.619  &  45.08  &   3575  & -13.67  & \nodata &  45.28  &   3439  & -13.72  & -15.87  \\
    J131116.87$+$142613.0  &  0.499  &  45.41  &   4444  & -13.55  & -15.25  &  45.57  &   3849  & -13.61  & -14.56  \\
    J131413.40$+$434416.5  &  0.608  &  45.21  &   2888  & -13.58  & -14.88  &  45.39  &   1636  & -13.97  & -14.95  \\
    J131430.78$+$130745.6  &  0.742  &  45.55  &   5110  & -13.65  & \nodata &  45.79  &   4142  & -13.69  & -15.05  \\
    J131459.85$+$505932.9  &  0.609  &  45.08  &   2190  & -14.13  & -14.88  &  45.26  &   1825  & -14.24  & -15.26  \\
    J131506.02$+$140319.6  &  0.654  &  45.68  &  13669  & -13.30  & -15.99  &  45.80  &   8133  & -13.51  & -16.07  \\
    J131706.98$+$473358.1  &  0.494  &  44.69  &  10137  & -13.99  & \nodata &  44.89  &   6225  & -14.14  & \nodata \\
    J131825.16$+$534055.6  &  0.582  &  45.09  &   4716  & -13.74  & -15.36  &  45.17  &   4079  & -14.07  & -15.57  \\
    J131831.23$+$031948.7  &  0.606  &  45.00  &   5454  & -13.97  & -15.84  &  45.23  &   3537  & -14.06  & -15.50  \\
    J131840.21$+$000735.3  &  0.492  &  44.80  &   2645  & -14.09  & -15.18  &  44.90  &   2258  & -14.25  & -15.45  \\
    J132048.68$+$510313.7  &  0.467  &  45.07  &   2619  & -13.82  & -15.00  &  45.19  &   3103  & -13.74  & -14.82  \\
    J132115.86$+$284719.5  &  0.549  &  45.45  &   2584  & -13.34  & -15.68  &  45.56  &   2047  & -13.70  & -14.77  \\
    J132502.63$+$650415.4  &  0.581  &  45.03  &   6028  & -13.77  & -15.55  &  45.27  &   5467  & -13.33  & -15.24  \\
    J132515.64$+$555906.5  &  0.638  &  45.22  &   3924  & -13.44  & -14.90  &  45.28  &   1909  & -13.91  & -14.75  \\
    J132518.85$+$661459.9  &  0.733  &  45.45  &   3237  & -13.56  & \nodata &  45.69  &   3202  & -13.73  & -14.87  \\
    J132748.62$+$653405.9  &  0.524  &  44.83  &   2418  & -13.85  & -15.33  &  45.05  &   2576  & -13.92  & -15.59  \\
    J132756.16$+$111443.7  &  0.611  &  45.17  &   6248  & -13.68  & -15.18  &  45.36  &   5466  & -13.73  & -14.78  \\
    J133302.20$+$584016.6  &  0.592  &  44.88  &   3640  & -13.87  & -16.34  &  45.06  &   3046  & -14.01  & -15.35  \\
    J133519.23$+$501505.1  &  0.570  &  45.15  &   4154  & -13.56  & -15.67  &  45.36  &   4009  & -13.61  & -14.87  \\
    J133526.01$-$010028.1  &  0.671  &  45.26  &   3162  & -13.83  & \nodata &  45.34  &   4129  & -13.97  & -15.12  \\
    J133719.31$+$594905.5  &  0.658  &  45.08  &   3370  & -13.76  & -15.25  &  45.17  &   2781  & -14.25  & -15.15  \\
    J133821.87$+$291445.8  &  0.648  &  45.45  &   3754  & -13.37  & -15.66  &  45.68  &   3277  & -13.75  & -14.68  \\
    J134207.39$+$041704.0  &  0.572  &  45.06  &   7241  & -13.71  & -16.03  &  45.16  &   3802  & -13.89  & -15.17  \\
    J134246.60$+$613435.5  &  0.484  &  44.79  &   3549  & -13.99  & -15.41  &  44.93  &   2087  & -14.06  & -15.56  \\
    J134642.37$+$591131.2  &  0.501  &  44.68  &   2822  & -14.11  & -15.37  &  44.80  &   2725  & -14.25  & -15.73  \\
    J134749.87$+$582109.4  &  0.646  &  45.47  &   7721  & -13.41  & -15.99  &  45.71  &   6056  & -13.29  & -15.14  \\
    J134934.31$-$004102.9  &  0.515  &  44.85  &   4820  & -13.79  & -15.76  &  45.08  &   4259  & -13.98  & -14.92  \\
    J134948.39$-$010621.8  &  0.599  &  45.59  &   2210  & -13.18  & -14.95  &  45.59  &   2746  & -13.58  & -15.18  \\
    J135459.65$+$405218.2  &  0.473  &  44.70  &   2649  & -14.06  & -15.42  &  44.80  &   2442  & -14.23  & -16.11  \\
    J135534.82$+$395910.1  &  0.505  &  44.83  &   2928  & -13.81  & -15.73  &  45.03  &   2517  & -13.94  & -16.33  \\
    J135611.20$+$483545.7  &  0.465  &  44.86  &   6672  & -13.68  & -16.23  &  45.09  &   5279  & -13.84  & -15.71  \\
    J135729.10$-$024738.0  &  0.600  &  45.19  &   3314  & -13.67  & \nodata &  45.43  &   3291  & -13.69  & -15.17  \\
    J135803.86$+$340254.1  &  0.541  &  44.79  &   7099  & -13.86  & -15.59  &  45.01  &   4848  & -13.93  & -15.25  \\
    J135825.33$+$641948.6  &  0.532  &  45.01  &   6993  & -13.76  & -16.16  &  45.23  &   6018  & -13.81  & \nodata \\
    J135925.82$+$354640.3  &  0.620  &  45.36  &   6385  & -13.82  & -15.53  &  45.51  &   3161  & -14.06  & -15.80  \\
    J140012.57$+$353930.7  &  0.518  &  44.80  &  13621  & -13.75  & -15.61  &  44.90  &   6137  & -13.80  & -16.55  \\
    J140104.88$+$004332.7  &  0.666  &  45.41  &   5461  & -13.49  & -16.06  &  45.54  &   3402  & -13.71  & -15.11  \\
    J140203.69$+$561047.9  &  0.520  &  44.84  &   3120  & -13.73  & -15.20  &  45.00  &   2816  & -13.92  & -14.80  \\
    J140447.81$+$053708.2  &  0.603  &  45.08  &   3707  & -13.79  & \nodata &  45.17  &   2199  & -14.13  & -15.59  \\
    J140849.94$+$344816.0  &  0.575  &  45.33  &   2734  & -13.37  & -15.20  &  45.54  &   3013  & -13.33  & -14.63  \\
    J140929.14$-$015717.7  &  0.638  &  45.13  &   7019  & -13.83  & -16.21  &  45.39  &   4799  & -13.81  & -15.19  \\
    J141057.73$+$643310.7  &  0.461  &  44.98  &   3155  & -13.71  & -15.15  &  45.16  &   3582  & -13.69  & -14.66  \\
    J141312.58$+$564113.3  &  0.669  &  45.38  &  10690  & -13.81  & -15.35  &  45.44  &   5466  & -14.12  & -16.00  \\
    J141334.49$+$355142.9  &  0.489  &  44.80  &   4649  & -13.86  & -15.71  &  44.93  &   3981  & -13.69  & -15.29  \\
    J141535.41$+$624505.7  &  0.555  &  44.79  &   5691  & -14.03  & -15.95  &  45.01  &   4481  & -13.99  & -16.01  \\
    J141735.09$+$642707.5  &  0.697  &  45.27  &   4703  & -13.68  & -15.69  &  45.50  &   3878  & -13.83  & -15.06  \\
    J141925.76$+$380249.1  &  0.509  &  44.90  &   5443  & -13.78  & -16.18  &  45.11  &   4127  & -13.76  & -15.40  \\
    J141956.72$+$373912.8  &  0.478  &  45.12  &   6324  & -13.56  & -15.83  &  45.31  &   5798  & -13.72  & -14.87  \\
    J142111.09$+$361353.1  &  0.689  &  45.42  &   3465  & -13.58  & -16.93  &  45.68  &   3052  & -13.81  & -14.99  \\
    J142240.36$-$010646.1  &  0.718  &  45.13  &   5762  & -13.75  & -15.78  &  45.44  &   3595  & -13.84  & -15.34  \\
    J142240.36$-$010646.1  &  0.718  &  45.35  &   5930  & -13.54  & -15.43  &  45.53  &   5059  & -13.71  & -14.76  \\
    J142322.27$+$443459.8  &  0.606  &  45.11  &   7505  & -13.88  & -16.45  &  45.27  &   4609  & -13.82  & -15.24  \\
    J142550.72$+$240403.4  &  0.653  &  45.33  &   8212  & -13.67  & -15.39  &  45.55  &   6303  & -13.79  & \nodata \\
    J142656.15$+$483415.6  &  0.656  &  45.30  &   6887  & -13.60  & -15.57  &  45.61  &   5499  & -13.66  & -15.27  \\
    J142656.55$+$602903.2  &  0.624  &  44.98  &   4984  & -13.79  & -15.71  &  45.18  &   4188  & -13.78  & -15.06  \\
    J142658.58$-$002056.3  &  0.628  &  45.41  &  14380  & -13.34  & -15.22  &  45.68  &   7732  & -13.15  & -14.78  \\
    J142758.73$+$324741.4  &  0.569  &  44.95  &   7430  & -13.87  & -15.42  &  45.14  &   6695  & -13.85  & -14.92  \\
    J142859.04$+$322506.8  &  0.627  &  45.01  &   3095  & -13.84  & -15.43  &  45.21  &   2338  & -14.05  & -15.02  \\
    J142945.12$+$322233.8  &  0.660  &  45.22  &   1962  & -13.99  & -15.18  &  45.30  &   2450  & -14.13  & -15.20  \\
    J143141.91$-$011330.7  &  0.659  &  45.12  &   7219  & -13.58  & \nodata &  45.34  &   5604  & -13.58  & \nodata \\
    J143141.91$-$011330.7  &  0.659  &  45.15  &   8273  & -13.74  & \nodata &  45.36  &   5805  & -13.58  & \nodata \\
    J143157.95$+$341650.2  &  0.715  &  45.48  &   4282  & -13.54  & -14.68  &  45.69  &   4322  & -13.61  & -14.56  \\
    J143517.71$+$634259.3  &  0.528  &  44.88  &   2887  & -13.89  & -15.07  &  45.01  &   1868  & -14.00  & -15.71  \\
    J143730.00$+$330309.7  &  0.548  &  44.79  &   2712  & -14.22  & -15.51  &  44.94  &   2709  & -14.43  & -15.73  \\
    J143736.41$+$615509.9  &  0.553  &  45.13  &   4232  & -13.60  & -15.19  &  45.35  &   3588  & -13.69  & -15.52  \\
    J144314.19$-$024722.1  &  0.677  &  45.40  &   2652  & -13.57  & \nodata &  45.60  &   2487  & -13.84  & -14.97  \\
    J144733.05$+$345506.7  &  0.661  &  45.61  &   3535  & -13.75  & -15.37  &  45.51  &   3150  & -13.95  & \nodata \\
    J144737.04$+$332006.4  &  0.498  &  44.80  &   6648  & -13.90  & -15.77  &  44.95  &   4992  & -14.03  & -15.16  \\
    J145224.68$+$452223.7  &  0.468  &  45.13  &   6545  & -13.35  & -16.40  &  45.37  &   5792  & -13.39  & -14.75  \\
    J145325.40$+$123704.4  &  0.541  &  45.12  &   4264  & -13.42  & -15.48  &  45.39  &   3691  & -13.51  & -14.76  \\
    J145406.42$+$382814.8  &  0.625  &  45.21  &   6325  & -13.69  & \nodata &  45.46  &   4334  & -13.83  & -15.84  \\
    J145427.17$+$401814.1  &  0.632  &  45.04  &   6129  & -13.77  & -15.84  &  45.28  &   5263  & -13.82  & -15.01  \\
    J145450.03$+$111434.5  &  0.467  &  45.18  &   3570  & -13.36  & -15.01  &  45.36  &   3238  & -13.52  & -14.54  \\
    J145542.92$+$424957.4  &  0.652  &  45.24  &   2364  & -13.86  & -15.81  &  45.42  &   2585  & -14.06  & -15.14  \\
    J145551.73$+$002703.4  &  0.603  &  45.08  &  12604  & -13.75  & -16.29  &  45.33  &  10117  & -13.49  & -15.12  \\
    J145748.07$+$414546.9  &  0.599  &  45.02  &   6586  & -13.77  & -15.77  &  45.28  &   3975  & -13.83  & -15.74  \\
    J145900.99$+$331919.9  &  0.494  &  44.76  &   7893  & -13.85  & -15.49  &  45.02  &   6474  & -13.84  & -15.31  \\
    J145958.43$+$333701.8  &  0.644  &  45.16  &   4692  & -13.50  & -15.54  &  45.39  &   4229  & -13.35  & -14.61  \\
    J150142.08$+$553809.7  &  0.545  &  45.01  &   4801  & -13.72  & -15.55  &  45.22  &   4622  & -13.72  & -14.73  \\
    J150257.98$+$502914.8  &  0.531  &  45.27  &   4399  & -13.51  & -15.23  &  45.49  &   3841  & -13.75  & -14.73  \\
    J150401.78$+$445911.1  &  0.493  &  45.16  &   3231  & -13.58  & -14.94  &  45.31  &   2809  & -13.75  & -14.79  \\
    J150751.68$+$602052.2  &  0.477  &  44.73  &   2483  & -14.02  & -15.77  &  44.87  &   2133  & -14.47  & -16.12  \\
    J150949.73$+$415538.9  &  0.573  &  45.14  &   2524  & -13.61  & -15.19  &  45.36  &   3847  & -13.61  & -14.56  \\
    J151140.34$+$402721.6  &  0.559  &  45.10  &   5090  & -13.53  & -16.63  &  45.25  &   3886  & -13.55  & -15.13  \\
    J151518.30$+$551535.4  &  0.514  &  44.97  &   5599  & -13.49  & -15.73  &  45.20  &   4050  & -13.56  & -15.07  \\
    J152017.24$+$313535.6  &  0.643  &  45.50  &   2350  & -13.53  & -14.84  &  45.63  &   1915  & -13.72  & -15.41  \\
    J152151.24$+$370153.2  &  0.561  &  44.92  &   7481  & -13.71  & -15.39  &  45.13  &   5661  & -13.49  & -15.62  \\
    J152544.33$+$563411.9  &  0.501  &  44.82  &   2390  & -13.84  & -14.88  &  45.07  &   2108  & -14.06  & -14.91  \\
    J152654.61$+$565512.4  &  0.482  &  44.86  &   2616  & -13.74  & -33.01  &  45.03  &   2399  & -13.86  & -16.18  \\
    J152816.62$+$322258.0  &  0.523  &  44.84  &   3430  & -13.77  & -15.29  &  45.06  &   2997  & -13.82  & -15.64  \\
    J152922.08$+$525247.3  &  0.634  &  45.08  &   5290  & -13.78  & -15.99  &  45.29  &   3939  & -13.72  & \nodata \\
    J153102.49$+$435637.6  &  0.452  &  45.11  &   2332  & -14.04  & -15.30  &  45.21  &   1816  & -14.18  & \nodata \\
    J153306.42$+$000635.2  &  0.589  &  44.94  &   4406  & -13.68  & -15.09  &  45.22  &   4417  & -13.70  & -14.93  \\
    J153600.36$+$483709.6  &  0.643  &  45.34  &   3608  & -13.79  & -15.68  &  45.46  &   3219  & -13.95  & -15.60  \\
    J153612.09$+$524154.6  &  0.561  &  45.26  &   2916  & -13.72  & \nodata &  45.51  &   2965  & -13.58  & \nodata \\
    J153715.34$+$023049.7  &  0.480  &  45.01  &   3568  & -13.51  & -15.23  &  45.16  &   2805  & -13.73  & \nodata \\
    J153733.20$-$005537.7  &  0.542  &  44.93  &   2070  & -13.71  & -15.80  &  45.16  &   2438  & -13.91  & -14.83  \\
    J153804.00$+$353658.5  &  0.525  &  44.95  &   4539  & -13.72  & -15.86  &  45.19  &   4479  & -14.09  & -15.02  \\
    J154115.80$-$014208.7  &  0.569  &  45.16  &   2667  & -13.74  & -14.94  &  45.22  &   2131  & -14.25  & -15.12  \\
    J154201.96$-$020649.6  &  0.482  &  44.94  &   4888  & -13.84  & -15.63  &  45.12  &   3383  & -13.83  & -15.14  \\
    J154342.46$+$461233.5  &  0.599  &  45.18  &   5471  & -13.64  & -15.67  &  45.35  &   6190  & -13.86  & -15.00  \\
    J154510.96$+$345246.9  &  0.516  &  45.27  &   2601  & -13.79  & -14.97  &  45.39  &   1928  & -14.06  & -14.96  \\
    J154843.66$+$290859.3  &  0.550  &  44.95  &   7150  & -13.73  & -15.29  &  45.10  &   8176  & -13.76  & -14.89  \\
    J155048.30$+$400144.9  &  0.497  &  45.14  &   4726  & -13.43  & \nodata &  45.38  &   4332  & -13.51  & -14.66  \\
    J155304.93$+$354828.6  &  0.723  &  45.77  &   2727  & -13.37  & -14.82  &  45.97  &   2131  & -13.67  & -14.86  \\
    J155346.77$+$362154.3  &  0.461  &  44.67  &   5730  & -13.67  & \nodata &  44.85  &   4605  & -13.45  & -15.68  \\
    J155435.23$+$324646.9  &  0.567  &  45.00  &   6033  & -13.65  & \nodata &  45.18  &   5830  & -13.63  & -14.88  \\
    J155837.78$+$081345.8  &  0.517  &  44.95  &   2514  & -13.62  & -15.56  &  45.10  &   2180  & -13.89  & \nodata \\
    J160141.31$+$262729.7  &  0.647  &  45.08  &   2836  & -13.88  & -15.40  &  45.35  &   2958  & -13.92  & -14.92  \\
    J160317.91$+$090037.9  &  0.489  &  44.69  &   9346  & -13.82  & -15.70  &  44.93  &   7448  & -13.74  & -16.05  \\
    J160715.70$+$401227.8  &  0.513  &  44.92  &   6098  & -13.74  & -15.37  &  45.07  &   4871  & -13.62  & -15.56  \\
    J161151.28$+$252028.7  &  0.556  &  45.00  &   4904  & -13.67  & -16.81  &  45.28  &   4119  & -13.57  & -15.22  \\
    J161246.98$+$451248.2  &  0.583  &  45.06  &   6112  & -13.75  & -15.76  &  45.21  &   4220  & -14.01  & -15.08  \\
    J161425.17$+$375210.8  &  0.552  &  45.24  &   5234  & -13.52  & -15.29  &  45.44  &   3536  & -13.70  & -14.72  \\
    J161428.07$+$493004.5  &  0.647  &  45.19  &   3542  & -13.79  & -16.57  &  45.39  &   3086  & -13.97  & -14.91  \\
    J161815.84$+$304705.8  &  0.720  &  45.35  &   3627  & -13.86  & -15.12  &  45.48  &   2879  & -14.01  & -15.13  \\
    J161916.55$+$334238.4  &  0.471  &  45.12  &   5362  & -13.44  & -15.30  &  45.32  &   4757  & -13.50  & -14.94  \\
    J161924.11$+$260907.3  &  0.629  &  45.33  &   2318  & -13.86  & -15.62  &  45.48  &   1969  & -14.04  & \nodata \\
    J162032.92$+$442249.5  &  0.585  &  45.19  &   2578  & -13.83  & -14.84  &  45.37  &   1969  & -14.06  & -15.72  \\
    J162032.92$+$442249.5  &  0.586  &  45.18  &   1900  & -13.86  & -15.67  &  45.37  &   2170  & -14.03  & -15.62  \\
    J162219.43$+$475132.4  &  0.640  &  45.25  &   6864  & -13.57  & -15.53  &  45.46  &   5038  & -13.63  & -14.78  \\
    J163334.40$+$290128.0  &  0.572  &  45.12  &   2936  & -13.61  & -15.03  &  45.29  &   2753  & -13.76  & -14.68  \\
    J163746.56$+$425449.7  &  0.544  &  45.09  &   3857  & -13.53  & -15.11  &  45.35  &   2899  & -13.76  & -14.97  \\
    J164025.03$+$464449.1  &  0.537  &  44.76  &   3697  & -14.01  & -15.95  &  44.94  &   2527  & -14.17  & \nodata \\
    J164258.82$+$394837.0  &  0.593  &  46.13  &   4365  & -13.78  & -16.03  &  46.07  &   4291  & -13.42  & -14.64  \\
    J164824.91$+$293831.3  &  0.593  &  45.10  &   5268  & -13.78  & -15.63  &  45.28  &   2944  & -14.00  & -14.93  \\
    J165005.48$+$414032.4  &  0.585  &  44.94  &   5244  & -13.89  & -15.52  &  45.05  &   3794  & -13.81  & -15.88  \\
    J165029.08$+$190908.6  &  0.659  &  45.29  &   3664  & -13.77  & -17.01  &  45.31  &   3034  & -14.07  & -15.39  \\
    J165051.57$+$362723.8  &  0.556  &  44.82  &   2353  & -14.04  & -15.54  &  45.03  &   2831  & -14.19  & -15.40  \\
    J165051.57$+$362723.8  &  0.556  &  44.78  &   2409  & -14.08  & -15.41  &  45.00  &   2422  & -14.14  & -15.85  \\
    J165722.09$+$395551.4  &  0.580  &  45.05  &   1844  & -14.16  & -16.23  &  45.14  &   2536  & -14.07  & -15.20  \\
    J165818.39$+$331951.0  &  0.716  &  45.38  &   4150  & -13.58  & -15.88  &  45.67  &   3975  & -13.61  & -14.75  \\
    J165904.37$+$313044.1  &  0.710  &  45.36  &   3154  & -14.00  & -15.60  &  45.59  &   2517  & -13.96  & -15.45  \\
    J170056.01$+$243928.2  &  0.509  &  44.98  &  14056  & -13.62  & -15.63  &  45.14  &   7069  & -13.40  & \nodata \\
    J170334.02$+$375410.8  &  0.534  &  44.99  &   4069  & -13.83  & -15.90  &  45.09  &   3644  & -13.97  & -15.12  \\
    J170518.81$+$240402.1  &  0.690  &  45.35  &   3440  & -13.63  & -16.90  &  45.59  &   3233  & -13.80  & \nodata \\
    J170524.76$+$340356.7  &  0.559  &  44.93  &   1755  & -13.83  & \nodata &  45.14  &   2216  & -14.08  & -14.99  \\
    J170533.71$+$644004.7  &  0.535  &  44.72  &   3366  & -13.98  & -15.75  &  44.91  &   3035  & -14.19  & -15.14  \\
    J171131.30$+$333543.4  &  0.470  &  45.21  &   1793  & -13.49  & -15.96  &  45.40  &   1531  & -13.83  & -16.05  \\
    J171334.04$+$595028.3  &  0.615  &  44.96  &   6075  & -14.06  & -15.77  &  45.17  &   5522  & -13.95  & \nodata \\
    J171352.43$+$584201.3  &  0.522  &  44.91  &   5125  & -13.85  & -15.73  &  45.04  &   3912  & -13.94  & -15.97  \\
    J172258.04$+$272542.1  &  0.511  &  44.76  &   3701  & -13.85  & -18.29  &  44.99  &   4360  & -13.84  & -15.00  \\
    J173348.82$+$585651.1  &  0.491  &  44.84  &   4280  & -13.90  & -15.58  &  45.02  &   3241  & -13.95  & -16.35  \\
    J203725.24$-$053747.0  &  0.681  &  45.19  &   4485  & -13.79  & \nodata &  45.46  &   3856  & -13.84  & -15.56  \\
    J203730.40$-$053013.4  &  0.537  &  45.21  &   6527  & -13.75  & \nodata &  45.40  &   3907  & -13.70  & -15.89  \\
    J205608.48$+$002928.1  &  0.481  &  45.06  &   7017  & -13.54  & -15.84  &  45.37  &   5137  & -13.56  & -14.80  \\
    J210001.25$-$071136.3  &  0.599  &  46.06  &   3964  & -12.81  & -14.52  &  46.29  &   2937  & -13.05  & -14.38  \\
    J212130.14$-$000527.1  &  0.585  &  45.28  &   2292  & -13.74  & -14.83  &  45.51  &   2236  & -13.89  & -15.87  \\
    J212501.21$-$081328.6  &  0.625  &  45.38  &  13569  & -13.51  & -15.90  &  45.52  &   9733  & -13.36  & \nodata \\
    J212715.34$-$062041.7  &  0.704  &  45.24  &   8051  & -13.68  & -15.18  &  45.47  &   6708  & -13.68  & -14.85  \\
    J212724.33$+$004718.2  &  0.716  &  45.58  &   3845  & -13.35  & -15.24  &  45.70  &   2871  & -13.90  & -14.84  \\
    J213139.51$-$073138.3  &  0.509  &  44.72  &   9664  & -14.13  & -17.03  &  44.87  &   6724  & -13.93  & \nodata \\
    J214313.98$+$004715.0  &  0.494  &  44.81  &   4284  & -13.88  & -15.84  &  44.91  &   3661  & -13.98  & -14.97  \\
    J214843.56$+$001054.6  &  0.673  &  45.26  &  11707  & -13.65  & -15.62  &  45.50  &   5774  & -13.60  & \nodata \\
    J215014.77$-$065314.4  &  0.590  &  45.34  &   3685  & -13.33  & \nodata &  45.59  &   3685  & -13.32  & -14.88  \\
    J221126.76$+$124458.2  &  0.486  &  44.77  &   5137  & -13.69  & -15.95  &  45.09  &   4552  & -13.64  & -14.96  \\
    J222708.31$+$133614.1  &  0.497  &  45.17  &  11647  & -13.64  & -15.70  &  45.39  &   6329  & -13.67  & -15.21  \\
    J222741.66$+$002838.6  &  0.555  &  45.04  &   3161  & -13.70  & -16.66  &  45.25  &   2676  & -13.88  & -16.08  \\
    J223109.08$-$080900.6  &  0.503  &  44.84  &   2832  & -13.72  & -15.58  &  45.10  &   2623  & -13.93  & -15.31  \\
    J223336.01$+$123158.1  &  0.463  &  45.05  &   4485  & -13.52  & \nodata &  45.22  &   4733  & -13.56  & -14.55  \\
    J223500.74$-$101216.8  &  0.553  &  45.01  &   3457  & -13.72  & -15.59  &  45.20  &   3133  & -13.74  & -16.13  \\
    J223533.08$-$081322.0  &  0.457  &  44.70  &   3897  & -13.95  & -15.34  &  44.88  &   3386  & -13.90  & -15.03  \\
    J224013.41$-$083628.7  &  0.580  &  44.93  &   3909  & -13.62  & -15.15  &  45.18  &   3785  & -13.59  & -15.05  \\
    J224655.58$-$084258.2  &  0.471  &  44.77  &   3257  & -13.71  & -15.85  &  44.99  &   3046  & -13.98  & -15.00  \\
    J225738.21$+$134045.5  &  0.594  &  45.24  &   4240  & -13.41  & -15.32  &  45.49  &   3970  & -13.53  & -14.75  \\
    J232900.86$+$141504.5  &  0.544  &  44.70  &   2445  & -14.18  & -15.37  &  44.98  &   1883  & -14.37  & -15.91  \\
    J233908.80$-$000637.8  &  0.482  &  44.90  &   6413  & -13.88  & -15.98  &  45.04  &   3225  & -13.92  & -15.17  \\
    J234145.51$-$004640.6  &  0.524  &  44.84  &   4752  & -13.65  & -15.28  &  45.05  &   3265  & -13.79  & -14.98  \\
    J234440.04$-$003231.7  &  0.503  &  44.91  &   3962  & -13.77  & -15.78  &  45.17  &   3045  & -13.87  & -15.66  \\
    J235324.08$+$000358.2  &  0.561  &  45.04  &   4354  & -13.70  & -16.28  &  45.28  &   3228  & -13.63  & \nodata \\

\enddata

\tablecomments{
Col. (1) Object name.
Col. (2) Redshift derived from the peak of [O\,III]~$\lambda 5007$.
Col. (3) Luminosity of the power-law continuum at 5100 \AA.
Col. (4) FWHM of broad H$\beta$.
Col. (5) Flux of the broad component of H$\beta$.
Col. (6) Flux of the narrow component of H$\beta$.
Col. (7) Luminosity of the power-law continuum at 3000 \AA.
Col. (8) FWHM of broad Mg\,II.
Col. (9) Flux of the broad component of Mg\,II.
Col. (10) Flux of the narrow component of Mg\,II.
Luminosities, fluxes, and FWHM are in units of erg~s$^{-1}$,
erg~s$^{-1}$~cm$^{-2}$, and km~s$^{-1}$,
respectively.
%\textit{Table 2 is available in its entirety
%via the link to the machine-readable table above. A portion is
%shown here for guidance regarding its form and content.}
}
\end{deluxetable}
\clearpage

